Appearance Matching Adapter for Exemplar-based Semantic Image Synthesis in-the-Wild

Exemplar-based semantic image synthesis generates images aligned with semantic content while preserving the appearance of an exemplar. Conventional structure-guidance models like ControlNet, are limited as they rely solely on text prompts to control appearance and cannot utilize exemplar images as input. Recent tuning-free approaches address this by transferring local appearance via implicit cross-image matching in the augmented self-attention mechanism of pre-trained diffusion models. However, prior works are often restricted to single-object cases or foreground object appearance transfer, struggling with complex scenes involving multiple objects. To overcome this, we propose AM-Adapter (Appearance Matching Adapter) to address exemplar-based semantic image synthesis in-the-wild, enabling multi-object appearance transfer from a single scene-level image. AM-Adapter automatically transfers local appearances from the scene-level input. AM-Adapter alternatively provides controllability to map user-defined object details to specific locations in the synthesized images. Our learnable framework enhances cross-image matching within augmented self-attention by integrating semantic information from segmentation maps. To disentangle generation and matching, we adopt stage-wise training. We first train the structure-guidance and generation networks, followed by training the matching adapter while keeping the others frozen. During inference, we introduce an automated exemplar retrieval method for selecting exemplar image-segmentation pairs efficiently. Despite utilizing minimal learnable parameters, AM-Adapter achieves state-of-the-art performance, excelling in both semantic alignment and local appearance fidelity. Extensive ablations validate our design choices. Code and weights will be released.: https://cvlab-kaist.github.io/AM-Adapter/

==> figures/1_motive.tex <==
\begin{figure*}[htb!]
    \centering
    \vspace{-20pt}
    \includegraphics[width=\textwidth]{figures/fig_1_motive.pdf} 
    \vspace{-20pt}
    \caption{\textbf{Effectiveness of our AM-Adapter:} semantic image synthesis results by (a) ControlNeXt~\cite{peng2024controlnext}, (b) IP-Adapter~\cite{ye2023ip} + ControlNet~\cite{zhang2023adding}, (c) Ctrl-X~\cite{lin2024ctrl}, and (d) \textbf{AM-Adapter}.} 
    % Compared to prior studies that often fail to capture local exemplar's appearance or struggle with finding accurate matching between exemplar image and target segmentation, our AM-Adapter precisely matches exemplars to targets in content-rich scenarios, preserving local details while maintaining alignment with the target structure.}
    \vspace{-10pt}
    \label{qual:intro}
\end{figure*}


==> supple/figures/cross_domain_setting.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{supple/figures/fig_cross_domain_setting_old.pdf} 
    \vspace{-20pt}
    \caption{\textbf{Cross Domain Setting.}}
    \vspace{-10pt}
    
    \label{supple:cross_domain}
\end{figure*}


==> supple/tables/dino_table.tex <==
\begin{table*}[t]
\small
% \centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|ccc|c|c}
    \toprule
    % \multirow{2}{*}{Methods} & \multirow{2}{*}{Training} & \multicolumn{4}{c|}{BDD100K~\cite{yu2020bdd100k}} \\
    \cmidrule(lr){3-9} BDD100K Comparison & ControlNet & ControlNeXt & FreeControl & Cross-Image Attention & Ctrl-X & ControlNet + IP-Adapter & \textbf{AM-Adapter(Ours)} \\
    
    %Self-sim $\downarrow$ & $I_{\mathrm{DINO}}$ $\uparrow$ & $I_{\mathrm{CLIP}}$ $\uparrow$  &CLIP-FID $\downarrow$ \\
    % \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    \midrule

    DINO [CLS] loss $\downarrow$ & 0.095 & 0.078 & 0.100 & 0.137 & \cellcolor{warmyellow}{0.063} & 0.072 & \textbf{\cellcolor{yzybest}{0.056} } \\
    $I_\text{DINO}$ $\uparrow$ & 0.654 & 0.695 & 0.479 & 0.495 & \cellcolor{warmyellow}{0.743} & 0.732 & \textbf{\cellcolor{yzybest}{0.765}} \\
    % Ctrl-X~\cite{lin2024ctrl}  &  0.051 & \cellcolor{yzybest}{0.788} & 0.700  & 45.75  \\

    % ControlNet~\cite{zhang2023adding} + IP Adapter~\cite{ye2023ip} & \cellcolor{warmyellow}{0.049} & 0.759 & \cellcolor{warmyellow}{0.805} & \cellcolor{yzybest}{15.35}  \\


    % \midrule
    % \bluerow \textbf{AM-Adapter (Ours)} &  \cellcolor{yzybest}{0.041} & \cellcolor{warmyellow}{0.786} & \cellcolor{yzybest}{0.819} & \cellcolor{warmyellow}{16.66}  \\
    \bottomrule
    \end{tabular}
    }
% \vspace{-5pt}
% \caption{\textbf{Quantitative comparisons.}}
% \label{tab:metric}
% \vspace{-10pt}
\end{table*}

==> supple/tables/quan_main.tex <==
% \begin{table*}[t]
% % \small
% \centering
% \begin{tabular}{l|c|ccc|ccc|}
% \toprule
% \multirow{4}{*}{Methods} & {Training} & \multicolumn{3}{c|}{BDD100K~\cite{}} & \multicolumn{3}{c|}{CityScapes~\cite{}}  \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}& & Self-sim $\downarrow$ & $I_{\mathrm{CLIP}}$ $\downarrow$ & FID $\downarrow$ & Self-sim $\downarrow$ & $I_{\mathrm{CLIP}}$ $\downarrow$ & FID $\downarrow$  \\
% % \cmidrule(lr){3-5}\cmidrule(lr){6-8}
% \midrule
% ControlNet~\cite{} + IPAdapter~\cite{} & \checkmark & -- & -- & -- & -- & -- & -- \\
% FreeControl~\cite{}  & \ding{55} & -- & -- & -- & -- & -- & -- \\
% Cross-Image Attention~\cite{}  & \ding{55} & -- & -- & -- & -- & -- & --  \\
% Ctrl-X~\cite{}  & \ding{55} & -- & -- & -- & -- & -- & -- \\
% % \midrule

% % \midrule
% \bluerow \textbf{Ours} & -- &  -- & -- & -- & -- & -- \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Quantitative comparisons.}}
% \label{tab:main}
% \end{table*}

\begin{table*}[t]
\small
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{l|l|ccc|ccc}
    \toprule
    \multirow{2}{*}{} & \multicolumn{1}{c|}{\multirow{2}{*}{ Methods}} & \multicolumn{3}{c|}{BDD100K~\cite{yu2020bdd100k}} & \multicolumn{3}{c}{CityScapes~\cite{cordts2016cityscapes}}  \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}& & Self-sim. $(\downarrow)$ & $I_{\mathrm{CLIP}}$ $(\uparrow)$  &FID $(\downarrow)$ & Self-sim. $(\downarrow)$ &  $I_{\mathrm{CLIP}}$ $(\uparrow)$ & FID $(\downarrow)$  \\
    % \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    % 
    \midrule
    &  Exemplar image & 0.052 & 1.000 & 44.23 & 0.049 & 1.000 & 40.00 \\
    \midrule 
    (I) & Pre-training & 0.047 & 0.731 & 94.48 & 0.055 & 0.760  & 130.04 \\
    (II) & (I) + MasaCtrl~\cite{cao2023masactrl}
     & 0.047  & \cellcolor{yzybest}{0.872} &  79.45 & 0.052 & \cellcolor{yzybest}{0.885} &  \cellcolor{yzybest}{81.37}  \\
    (III) & (I) + DreamMatcher~\cite{nam2024dreammatcher}
    &  0.046 &0.724  &79.34 & 0.061  & 0.776  &97.93\\
    
    \midrule
    (IV) & (I) + Augmented Self-Attention & 0.043 & 0.815  & 78.13 & \cellcolor{warmyellow}{0.048} & 0.830& 115.89 \\ 
    (V) & (IV) + w/ Fine-tuning & \cellcolor{softyellow}{0.043} & 0.808 & \cellcolor{softyellow}{77.75} & 0.051 & 0.810 & 134.00 \\ 
    (VI) & (IV) + Categorical Matching Cost & \cellcolor{warmyellow}{0.043} & \cellcolor{softyellow}{0.817} & \cellcolor{warmyellow}{76.76} & \cellcolor{softyellow}{0.050} & 
    \cellcolor{softyellow}{0.832} & \cellcolor{softyellow}{96.36} \\
    \midrule 
    % (VII) & AM-Adapter (Ours) w/o matching guidance. & -- & -- & -- & -- & -- & -- \\
    (VII) &  \textbf{AM-Adapter (Ours)} &   \cellcolor{yzybest}{0.041}  & \cellcolor{warmyellow}{0.819} & \cellcolor{yzybest}{75.89} & \cellcolor{yzybest}{0.048} & \cellcolor{warmyellow}{0.835}  & \cellcolor{warmyellow}{85.67} \\
    \bottomrule
    \end{tabular}

}

\caption{\textbf{Quantitative Comparison.} Although the table displays scores rounded to three decimal places, we determine the rankings based on precision to the fourth decimal place.}
\label{tab:quan_main}
\end{table*}

% \begin{table*}[t]
% \small
% \centering
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|c|cccc|cccc}
%     \toprule
%     \multirow{2}{*}{Methods} & \multirow{2}{*}{Training} & \multicolumn{4}{c|}{BDD100K~\cite{yu2020bdd100k}} & \multicolumn{4}{c|}{CityScapes~\cite{cordts2016cityscapes}}  \\
%     \cmidrule(lr){3-6}\cmidrule(lr){7-10}& & Self-sim $\downarrow$ & $I_{\mathrm{DINO}}$ $\uparrow$ & $I_{\mathrm{CLIP}}$ $\uparrow$  &CLIP-FID $\downarrow$ & Self-sim $\downarrow$ & $I_{\mathrm{DINO}}$ $\uparrow$ & $I_{\mathrm{CLIP}}$ $\uparrow$ & CLIP-FID $\downarrow$  \\
%     % \cmidrule(lr){3-5}\cmidrule(lr){6-8}
%     \midrule
%     ControlNet~\cite{zhang2023adding} 
%     & \checkmark & 0.052 & 0.658 & 0.638 & 57.19 & 0.058 & 0.702 & 0.761 & 48.11  \\
%     ControlNext~\cite{peng2024controlnext}  
%     & \checkmark & 0.047 & 0.716 & 0.731 & 20.97 & 0.055 & 0.737 & 0.760 & 33.62  \\
%     \midrule
%     FreeControl~\cite{mo2024freecontrol}  & \ding{55} & 0.062 & 0.530 & 0.575 & 65.64 & 0.073 & 0.573 & 0.690 & 48.69  \\
%     Cross-Image Attention~\cite{alaluf2024cross}  & \ding{55} & 0.177 & 0.557 & 0.643  & 64.25 & 0.133 & 0.658 & 0.754 & 45.74   \\
%     Ctrl-X~\cite{lin2024ctrl}  & \ding{55} & 0.051 & \cellcolor{yzybest}{0.788} & 0.700  & 45.75 & 0.058 & \cellcolor{yzybest}{0.809} & 0.818 & 26.10 \\
%     \midrule

%     ControlNet~\cite{zhang2023adding} + IP Adapter~\cite{ye2023ip} & \checkmark & \cellcolor{warmyellow}{0.049} & 0.759 & \cellcolor{warmyellow}{0.805} & \cellcolor{yzybest}{15.35} & \cellcolor{warmyellow}{0.049} & 0.783 & \cellcolor{warmyellow}{0.823} & \cellcolor{yzybest}{17.46}  \\
%     %ControlNet~\cite{zhang2023adding} + DreamMatcher~\cite{nam2024dreammatcher} & \checkmark & \cellcolor{warmyellow}{0.049} & 0.759 & \cellcolor{warmyellow}{0.805} & \cellcolor{warmyellow}{84.82} & \cellcolor{warmyellow}{0.049} & 0.783 & \cellcolor{warmyellow}{0.823} & 115.98  \\
    
%     \midrule
%     \bluerow \textbf{AM-Adapter (Ours)} & \checkmark &  \cellcolor{yzybest}{0.041} & \cellcolor{warmyellow}{0.786} & \cellcolor{yzybest}{0.819} & \cellcolor{warmyellow}{16.66} & \cellcolor{yzybest}{0.048} & \cellcolor{warmyellow}{0.800} & \cellcolor{yzybest}{0.835}  & \cellcolor{warmyellow}{21.90} \\
%     \bottomrule
%     \end{tabular}

% }
% \vspace{-5pt}
% \caption{\textbf{Quantitative comparisons.}}
% \label{tab:main}
% \vspace{-10pt}
% \end{table*}

